The Computational Power of Distributed Shared-Memory Models with Bounded-Size Registers

The celebrated Asynchronous Computability Theorem of Herlihy and Shavit (STOC 1993 and STOC 1994) provided a topological characterization of the tasks that are solvable in a distributed system where processes are communicating by writing and reading shared registers, and where any number of processes can fail by crashing. However, this characterization assumes the use of full-information protocols, that is, protocols in which each time any of the processes writes in the shared memory, it communicates everything it learned since the beginning of the execution. Thus, the characterization implicitly assumes that each register in the shared memory is of unbounded size. Whether unbounded size registers are unavoidable for the model of computation to be universal is the central question studied in this paper. Specifically, is any task that is solvable using unbounded registers solvable using registers of bounded size? More generally, when at most $t$ processes can crash, is the model with bounded size registers universal? These are the questions answered in this paper.

==> 1resilient_simulation.tex <==
\section{OLD SECTION: (unfinished) simulation with constant size registers }
\label{sec:universality}


\subsection{$1$-resilient computations}
\label{sec:1-resilient-comp}
In this section we establish that any task that can be solved with
unbounded  registers while tolerating at most one failure by $n$
processes can also be solved with $n$ constant-size communication SWMR
registers. The size of the registers does not depend on the task nor
on the number of processes. More precisely, this section is devoted to the proof of
the next theorem: 

\begin{theorem}
  \label{thm:1_resilient_universality}
  There exists $s \in \mathbb{N}$ such that for any
  task $T$ and any number of processes $n \geq 2$,  $T$ solvable $1$-resilient by $n$ processes  using unbounded registers  $\implies$ $T$  
  solvable $1$-resilient with $n$ input SWMR registers and $n$
  computation SWMR registers of size  $s$.  
\end{theorem}


\subsubsection{Overview }Let $n \geq 3$ and let $T = (\m{I},\m{O},\Delta)$ be a task that is $1$-resiliently solvable by
$n$ processes. Biran, Moran and Zaks~\cite{BMZ90charac} give necessary
and sufficient conditions for tasks to be solvable
$1$-resiliently. Essentially,  solving $T$ boils down for the
processes to select an edge in a graph  induced by the
possible outputs of the task. More precisely, as $t=1$, processes may
have at most two views of inputs in a an execution: A \emph{full input
vector} $x$ consisting of every input and a \emph{partial input vector} $x^j$ in
which the input of one process $j$ is missing.  It is shown
in~\cite{BMZ90charac} that  $\m{O}$ induces an \emph{output graph}
$G_\m{O}$ whose nodes are \emph{full output vectors}; each full input
vector  $x$ (respectively, partial input vector  $x^j$) can  be mapped
to a node $\delta(x)$  (respectively $\delta(x^j)$) in such a way that
there is path $path(\delta(x),\delta(x^j)) = (y_0,\ldots,y_L)$
connecting $\delta(x)$ and $\delta(x^j)$. Moreover, each node $y_\ell$
in this path is valid output for $x$, and any adjacent nodes differ
in at most one entry. Therefore, processes may solve $T$ by each selecting
a vertex in $path(\delta(x),\delta(x^j))$ such that chosen vertexes
form an edge in the path. This in turn can be achieved using an
$\epsilon$-agreement protocol with $\epsilon =
\frac{1}{L+1}$. A process seeing the full input $x$ starts with $0$,
or $1$ if it sees a partial input $x^j$. After getting back a decision
$d = k\epsilon$ from the protocol, it selects vertex
$y_{\frac{d}{\epsilon}}$ in the path $path(\delta(x),\delta(x^j))$. The
path can be inferred by having processes writing to shared memory
their view of the inputs before invoking the $\epsilon$-agreement
protocol and, since the decisions are the same or $\epsilon$ apart,
a single vertex or an edge is collectively chosen by the processes.

Section~\ref{sec:epsilon_agreement} presents a wait-free $\epsilon$-agreement
protocol $\m{A}_R$ using 2 constant-size communication register. With the
BG-simulation~\cite{BorowskyGLR01}, $n$ processes can simulate
executions of $\m{A}_R$ tolerating $1$ failures. However, the
BG-simulation requires registers of unbounded size. Another challenge
concerns the communication of the (partial) views of the inputs that
define the path on which vertexes are selected, as the size of inputs
of $T$ is arbitrary. 

Our simulation keeps the general structure of the BG-simulation and
uses as building blocks specially crafted safe-agreement objects. We
additionally exploit the structure of the simulated algorithm
$\m{A}_R$ to \emph{recycle} safe-agreement objects: a safe-agreement
object used for the simulation of round $r$ of $\m{A}_R$ can be reused
to simulate round $r+c$, where $c$ is a constant independant of $n$
and $\epsilon$.



\subsubsection{Characterization of 1-resilient solvable tasks}
We assume that the number of processes $n$ is at
least $3$.  Biran, Moran and Zaks~\cite{BMZ90charac} give necessary
and sufficient conditions for a task to be solvable $1$-resiliently in
the asynchronous message passing model. When at most one process may
fail and  $n\geq 3$, any shared memory $1$-resilient algorithm that
uses  only registers can be simulated in the message-passing
model~\cite{AttiyaBD95}. Reciprocally, it is easy to simulate a
message-passing algorithm using  registers. Hence, the
conditions of~\cite{BMZ90charac} also characterize the tasks that are
$1$-resilient solvable using  registers.


We recall the main ingredients of the characterization
of~\cite{BMZ90charac}. Let $T = (\m{I},\m{O},\Delta)$ be a task for
$n$ processes. 
% A \emph{task} $T$ for $n$-processes is a triplet $T =
% (\m{I},\m{O},\Delta)$  where $\m{I}$ and $\m{O}$ are sets of size $n$ vectors  over some
% finite sets of values (e.g., $\m{I} \subseteq \m{V}^n, \m{O} \subseteq
% \m{W}^n$  where $\m{V}$ and $\m{W}$ are finite sets) and the relation
% $\Delta \subseteq \m{I}\times \m{O}$ defines for each input vector $I
% \in \m{I}$ which outputs $O \in \m{O}$ the processes are collectively
% allowed to decide.
As we are concerned with $1$-resilient computation,
a process may fail before deciding or writing  its input to a shared
register. This is modelled in~\cite{BMZ90charac}  by considering
$n$-components input and output vectors where
at most one entry is missing. We say that a vector $c \in (\m{V} \cup \bot)^n$ is
\emph{full} if $\forall i, 1\leq i \leq n$, $c[i] \neq \bot$ and
\emph{partial} if there exists a unique index $j$ such that $c[j] =
\bot$.  Given a full vector $c$, let $c^j$ be  the vector $c$ in which
the $j$th entry is replaced by $\bot$.  $c$ is called an
\emph{extension} of $c^j$. 

Given a set $\m{Y}$ of full output vector, $G(Y)$ is the graph whose
set of nodes is $\m{Y}$ and there is an edge between two nodes $y$ and
$y'$ if and only if there is an unique $j$ such that $y[j] \neq
y'[j]$. Task $T$ is $1$-resilient solvable if and only if there exists
a restriction $\m{O'} \subseteq \m{O}$ of the outputs satisfying:
\begin{enumerate}
\item  (\emph{connectivity}) for any full input $x \in \m{I}$, the graph
$G(\Delta(x) \cap \m{O'})$ is connected and,
\item  (\emph{covering}) For any partial input vector $x^j$, there
  exists a partial output vector $y^j$ such that for extension $x$ of
  $x^i$, there is an extension $y \in \Delta(x) \cap \m{O}'$ of $y^j$.  
\end{enumerate}

We next define a map $\delta$ from full and partial input vectors to 
output vector as follows:
\begin{itemize}
\item For a full input vector, $\delta(x)$ is an arbitrary full output
  vector in $\Delta(x) \cap \m{O}'$
\item For a partial a partial input vector $x^i$, let $y^i$ be a partial
  output vector that, for each extension $x$ of $x^i$,  has a valid
  extension $y \in \Delta(x) \cap \m{O}'$. The existence of $y^i$ is
  guaranteed by the covering condition above. We set $\delta(x^i) = y^i$. 
\end{itemize}
We now ague that there is path from $\delta(x)$  to $\delta(x^i)$ in
$G(\Delta(x) \cap \m{O}' \cup \{\delta(x^i))$. By the connectivity
condition, since $x$ extends $x^i$, there exists $y$ extension of $y^i
= \delta(x^i)$ in $\Delta(x) \cap \m{O}'$. $y$ and $y^i$ are connected
since they differ only their $i$th entry. As $y$ and $\delta(x)$ are
both valid output for $x$ in $\m{O'}$, there is a path that connects
them in $G(\Delta(x) \cap \m{O}'$ by the connectivity condition. We
denote by $path(\delta(x),\delta(x^i))$ such a path. Note that every
node in the path except $\delta(x^i)$ is a valid  full output vector
for $x$, and $\delta(x^i)$ a valid partial output vector for
$\delta(x^i)$. Suppose that  $y_\ell$ and $y_{\ell+1}$
are adjacent nodes in $path(\delta(x),\delta(x^i))$. They differ in
one entry $k$. Suppose that in some algorithm for $T$, in an execution
with input vector $x$, each process chooses its  output in $y_\ell$ or
$y_{\ell+1}$. Let us observe that depending of the choice of process $k$, the full output
vector is either  $y_\ell$ or $y_{\ell+1}$ which belongs to
$\Delta(x)$. 

In the following, we assume that $\delta$ is fixed and, for simplicity,
that every path $(path(\delta(x)),path(\delta(x^i)))$ has the same
length $L$. This can be achieved by adding adjacent copies of one of
the nodes in shorter paths.
% Essentially, it is shown in~\cite{BMZ90charac} that solving a task
% $T=(\m{I},\m{O},\Delta)$ $1$-resilient boils down to agree on an edge
% in a path formed by output vectors. The path is induced by views 
% input vector $x$ and a partial vector $x^j$. Indeed, 

% Given a path
% $(y_0,\ldots,y_L)$ agreeing on a edge means that each process has to
% select one a vertex $y$ in path such that the set of selected vertexes
% form an edge in the path. Assuming that the path is known by the
% processes, this is turn can be achieved using an $\epsilon$-agreement
% protocol with $\epsilon = \frac{1}{L+1}$.  Each process $i$ starts with
% $0$ or $1$, corresponding to the ends of the path, and after getting
% a decision  $d_i$  from the $\epsilon$-agreement protocol, outputs
% the vertex $y_{\frac{d_i}{\\epsilon}}$.
% Since \textbf{HEREH HERHEH}.

\subsubsection{Safe agreements}
Our simulation relies, as the BG-simulation, on \emph{safe agreement}
objects as building blocks to agree on the steps of the two simulated
processes. Different specifications of safe agreement
 can be found in the literature, e.g.,
\citetodo{Attiya06,BorowskyGLR01,ImbsR09}. Our specifications is
closed to \citetodo{Attiya06}. 
 
A safe agreement object supports two operations $\mathsf{propose}(v)$
where $v$ is a value in some finite domain $D$ and
$\mathsf{decide}()$. Each
process is required to  invoke
$\mathsf{propose}()$ at most once, while $\mathsf{decide}()$ can be
invoked arbitrarily many times. $\mathsf{propose}()$ returns nothing while
$\mathsf{decide}()$ returns a value in $D \cup \{\bot\}$ satisfying: 
\begin{enumerate}
\item\label{sa:val} \emph{Validity}. If a $\mathsf{decide}()$ operation returns  value
  $v \neq \bot$,  $v$ is the input of a $\mathsf{propose}()$ operation.
\item\label{sa:agr} \emph{Agreement}. If values $v \neq \bot,v' \neq \bot$ are
  returned by $\mathsf{decide}()$ operations, $v = v'$.
\item\label{sa:term} \emph{Termination}. Every operation performed by
  a non-faulty process terminates.
\item\label{sa:cons} \emph{Consistent decisions}. 
  If a  $\mathsf{decide}()$ operation returns $v \neq \bot$, every
  $\mathsf{decide}$ operation that follows returns a non-$\bot$ value.
  \item\label{sa:nontriv} \emph{Non triviality}. In some executions
    (specified later), if $\mathsf{decide}()$ operations are performed
    infinitely often, at least one of them returns a non-$\bot$ value.  
\end{enumerate}
A safe agreement object is said to be \emph{decide} after a
$\mathsf{decide}$ operation has returned a non-$\bot$ value and
\emph{undecided} otherwise.

We use safe-agreement objects to simulate two processes $A$ and $B$
executing the $\epsilon$-agreement protocol $\m{A}_R$
(Section~\ref{sec:epsilon_agreement}) and for agreeing on (partial)
vectors $\delta(x), \delta(x^j)$. We present next  implementations of safe
agreement with slightly different non-triviality conditions tailored
for different purpose: Input Agreement A (\emph{IAA},
Algorithm~\ref{alg:IAA}) and Input Agreement B (\emph{IAB},
Algorithm~\ref{alg:IAB}) for determining the two end points
$\delta(x)$ and $\delta(x^i)$ on the path on which a single vertex or
an edge has to be selected; Safe Agreement A (\emph{SAA},
Algorithm~\ref{alg:SAA}) and Safe Agreement B (\emph{SAB},
Algorithm~\ref{alg:SAB}) for agreeing on the steps of processes $A$
and $B$ in the simulation. 
Each implementation is very simple or a minor variation of an existing
implementation. All of our implementation uses $n$ SWMR registers of
constant size (independant of $n$ and $\epsilon$).

\paragraph{Notations}
We denote by $\#_{val}(X)$  the number of occurrences of $val$ in
vector $X$. $n$ is the number of (simulator) processes. $T =
(\m{I},\m{O},\Delta)$ is the task the processes want to solve
tolerating $1$ failures.   

\paragraph{Agreeing on (partial) input vectors}
The values output by the simulation of the $\epsilon$-agreement
algorithm are used to select nodes in a path $path(y_A,y_B) =
path(\delta(x),\delta(x^i))$. The purpose of 
Algorithms~\ref{alg:IAA} and Algorithm~\ref{alg:IAB} is for the
simulator processes to agree on the end points of this path.
Before invoking $\textsc{propose}()$, each process must have written its input for $T$
its dedicated input register $I[i]$.  While  a
process may repeatedly read $I$  until seeing $n-1$ inputs as at most
one process may fail, it  cannot communicate the  index of the missing
input as this would require communication registers of size $O(\log
n)$. 



In Algorithm~\ref{alg:IAA}, $\textsc{propose}()$ takes no input and
consists for process $i$ in writing $\mathtt{H}$ (for 'here') in its
communication register $R[i]$ (line~\ref{iaa:propose}). $\textsc{decide}()$ returns a copy of
$I$ once every process has written $\mathtt{H}$ to $R$, and $\bot$
otherwise (lines~\ref{iaa:return_inputs}-\ref{iaa:return_bot}). The
properties of Algorithm~\ref{alg:IAA} are summarized in the next
Lemma:
\begin{lemma}
  \label{lem:iaa}
  Algorithm~\ref{alg:IAA} satisfies agreement, termination, consistent
  decisions of safe agreement and
  \begin{itemize}
  \item non-triviality: if every process invokes $\textsc{propose}()$ and each
    invocation terminates, only finitely many invocations of
    $\textsc{decide}()$ return $\bot$. 
  \item validity: if a $\textsc{decide}()$ operation returns $v \neq
    \bot$ then $v$ is a full $n$-components vector corresponding to
    the inputs of the processes. 
  \end{itemize}
\end{lemma}


\begin{algorithm}
  \caption{IAA : Input Agreement for simulated process A. Code for process $i$. Before invoking $\textsc{propose}()$ or $\textsc{decide}()$, process $i$ must have written its input to the array of input register $I$.}
  \label{alg:IAA}
  \begin{algorithmic}[1]
    \Statex \textbf{shared variables} $R[1..n]$ array of $n$ 2-valued registers, initially $[\bot,\ldots,\bot]$   
    \Function{propose}{$~$}\label{iaa:propose}
    \State\label{iaa:writeH}$R[i].\mathsf{write}(\mathtt{H})$ 
    \EndFunction
    \Function{decide}{$~$}\label{iaa:decide}
    \State\label{iaa:collect}$c \gets R.\mathsf{collect}()$;
    \If{$\#_0(\bot) = 0$}\label{iaa:return_inputs} $\mathit{inputs} \gets I.\mathsf{collect}()$;  
 \textsl{return} $\mathit{inputs}$ \Else{}\label{iaa:return_bot} \textsl{return} $\bot$
    \EndIf
    \EndFunction
  \end{algorithmic}
\end{algorithm}

In Algorithm~\ref{alg:IAB}, $\textsc{propose}()$ takes no inputs and
$\textsc{decide}()$ returns $\bot$, a partial or a full input
vector. When it performs $\textsc{propose}()$, process $i$ first
announces itself by writing $\mathtt{H}$ to $R[i]$. It then waits
until at least $n-1$ processes have written to $R$. %The additional
%$\mathsf{collect}()$ at line~\ref{iab:2ndcollect} ensures that
%every partial collected vector $c$ (with one $\bot$ entry) are the
%same.
Depending on whether or not its view $c$ of $R$ contains one
$\bot$ component, it then writes in $R[i]$ $\mathtt{F}$ (for full) or
$\mathtt{P}$ (for partial).  Note that not all processes can write $\mathtt{P}$. Indeed, the  process $\ell$ that last writes $\mathtt{H}$ to $R$ reads a non-$\bot$ value in each registers $R[1],\ldots,R[n]$ and therefore does not write $\mathtt{P}$ to $R[\ell]$. 

A $\textsc{decide}()$ operation by process $i$ returns the full
vector corresponding the  processes input to task $T$ if $i$ sees at
least two occurrences of 
$\mathtt{F}$ in $R$ (line~\ref{iab:return_full}),  a partial vector
(line~\ref{iab:return_partial}) if there are $n-1$ occurrences of
$\mathtt{P}$, and $\bot$ otherwise~\ref{iab:return_bot}. As once a
process  $\mathtt{F}$ or $\mathtt{P}$ has been written to a register
$R[j]$, the value of that register never changes,
line~\ref{iab:return_full} and line~\ref{iab:return_partial} are
mutually exclusive. This ensures that the implementation satisfies
agreement and consistent reads. An invocation of $\textsc{decide}$
returns a non-$\bot$ value once $\textsc{propose}()$ has been invoked
by $n-1$ or $n$ processes, and each invocation has terminated. To
summarize:
\begin{lemma}
  \label{lem:iab}
  Algorithm~\ref{alg:IAB} satisfies agreement, consistent
  decisions of safe agreement and
  \begin{itemize}
  \item termination: if     $\textsc{propose}()$ is invoked by at
    least $n-1$ non-faulty processes, every operation by  processes
    terminates. 
  \item non-triviality: if at least $n-1$ processes invokes $\textsc{propose}()$ and each
    invocation $of \textsc{propose}()$ terminates, only finitely many invocations of
    $\textsc{decide}()$ may return $\bot$. 
  \item validity: Let $x$ be the full input vector of the processes
    for $T$.  If a $\textsc{decide}()$ operation returns $v \neq
    \bot$ then $v = x$ or $v = x ^j$ for some $j, 1 \leq j \leq n$. 
  \end{itemize}
\end{lemma}
\begin{proof}
  \begin{itemize}
  \item Termination. Clearly, if $n-1$ or more non faulty processes
    invoke $\textsc{propose}()$, $R$ eventually stores  $0$ or $1$
    occurrences of $\bot$ and therefore every non-faulty process
    eventually exits the $\mathbf{repeat}$ loop of
    line~\ref{iab:repeat}. As the rest of the code of
    $\textsc{propose}()$  is wait-free, and so is the code of
    $\textsc{decide}()$ every operation by non-faulty processes
    terminates. 
  \item Validity. As observed in the description of the algorithm, at
    most $n-1$ occurrences of $\mathtt{P}$ are stored in $R$.  Hence
    the index $j$ at line~\ref{iab:return_partial} is well
    defined. Moreover, before writing $\mathtt{P}$ to $R[i]$, process
    $i\neq j$ has previously written its  input to $I[i]$. Therefore,
    each entry $i\neq j$ of the
    vector $inputs$ collected from $I$ at line~\ref{iab:collect_inputs} 
    contains a non-$\bot$ value. It thus follows that the
    vector returned at line~\ref{iab:return_partial} is the vector of
    inputs of the processes for $T$ with one entry $j$ replaced by $\bot$. 
  \item Agreement and consistent decisions. For any $i, 1 \leq i \leq n$, once $R[i]$ contains
    $\mathtt{P}$ or $\mathtt{F}$, its value never changes. Therefore
    it is not possible for one process to collect $\geq n-1$ occurrences
    of $\mathtt{P}$ in $R$ and $\geq 2$ occurrences of $\mathtt{F}$
    for another and agreement follows. When a $\textsc{decide}()$
    operation returns a vector $x \neq \bot$, there are at least $2$
    occurrences of $\mathtt{F}$ or at least $n-1$ occurrences of
    $\mathtt{P}$ in $R$. As this cannot change, any subsequent
    $\textsc{decide}()$ operation returns $x$. 
  \item Non-triviality. Suppose that every invocation of
    $\textsc{propose}()$ terminates and that 
    $\textsc{propose}()$ is invoked by at least $n-1$
    processes.

    If $\textsc{propose}()$ is invoked $n-1$ times, no
    $\mathtt{F}$ is ever written to $R$, and as these invocations
    terminates, eventually $R$ contains $n-1$ occurrences of
    $\mathtt{P}$. Therefore, eventually every $\textsc{decide}()$
    operation returns a ono-$\bot$ value at
    line~\ref{iab:return_partial}.

    If $\textsc{propose}()$ is invoked $n$ times, the value of
    each register $R[i], 1 \leq i \leq n$ is eventually $\mathtt{F}$
    of $\mathtt{P}$. Therefore, eventually every  vector $c$ collected
    from $R$ satisfies the condition of line~\ref{iab:return_partial}
    or line~\ref{iab:return_full}. 
  \end{itemize}
\end{proof}

\begin{algorithm}
  \caption{IAB : Input Agreement for simulated process B.  Code for process $i$. Before invoking $\textsc{propose}()$ or $\textsc{decide}()$, process $i$ is required to have written its input to the input array  $I$.}
  \label{alg:IAB}
  \begin{algorithmic}[1]
    \Statex   \textbf{shared variables} $R[1..n]$ array of $n$ 4-valued registers, initially $[\bot,\ldots,\bot]$ 
    \Function{propose}{$~$}\label{iab:propose}
    \State\label{iab:writeH}$R[i].\mathsf{write}(\mathtt{H})$
    \State\label{iab:repeat}\textbf{repeat} $c \gets R.\mathsf{collect}()$ \textbf{until} $\#_\bot(c) \leq 1$
%    \State\label{iab:2ndcollect}$c \gets R.\mathsf{collect}()$ not
%    needed ?
    \State\textbf{if} $\#_\bot(c) = 0$\label{iab:writeF}
    $R[i].\mathsf{write}(\mathtt{F})$ \textbf{else}\label{iab:writeP} $R[i].\mathsf{write}(\mathtt{P})$
    \EndFunction
    \Function{decide}{$~$}\label{iab:decide}
    \State\label{iab:decide_collect}$c \gets R.\mathsf{collect}()$; \label{iab:collect_inputs}$inputs \gets I.\mathsf{collect}()$
    \Case{$\#_{\mathtt{P}}(c) \geq n-1$} \label{iab:return_partial}
    let $j$: $c[j] \neq \mathtt{P}$; $inputs[j] \gets \bot$;
    \textsl{return} $inputs$
    \Statex\Comment{Partial input vector with
      one $\bot$-entry}
    \StateCase{$\#_\mathtt{F}(c) \geq 2~~~~~\ $}\label{iab:return_full}  \textsl{return} $inputs$  \Comment{Full input vector, no $\bot$-entry}
    \StateCase{\emph{default}$~~~~~~~~~~$}\label{iab:return_bot} \textsl{return} $\bot$
    \EndCase
    \EndFunction
  \end{algorithmic}
\end{algorithm}


\paragraph{Agreeing on  the views  of $A$ and $B$ }
An execution of $\m{A}_R$ proceeds in a asynchronous rounds. In a
round $r$, each process $P \in \{A,B\}$ writes a bit ($= r\mod 2$) in
its communication register $R[P]$. It then reads the register of the
other process. Based on its \emph{view}, obtained by reading the
register of the other process, it \emph{continues} to the next round
or \emph{stops} and decides.  The simulation consists
for the simulators to agree on the successive views of $A$ and
$B$. Instances of algorithms Algorithm~\ref{alg:SAA} (SAA) and
Algorithm~\ref{alg:SAB} (SAB) are used to agree on a view for $A$ and
$B$ respectively. We identify views we the same bit in the two
registers with $\mathtt{CONTINUE}$ (as in this case the simulated
process moves to the next round), and views with distinct  bits with
$\mathtt{STOP}$. 

 Algorithm~\ref{alg:SAA} is used to proposes a view at some round for
$A$. It is similar to Algorithm~\ref{alg:IAA}. To
proposes a view $v \in \{\mathtt{CONTINUE},\mathtt{STOP}\}$ for $A$,
process $i$ writes $v$ to $R[i]$. A $\textsc{decide}$ operation
return a view $w \neq \bot$ if and only if each process has written
its proposal to $R$. The decision returned by the operation is then
the proposal with the largest number of occurrences, or
$\mathtt{STOP}$ in case of a tie (line~\ref{saa:return_maj}).  


\begin{algorithm}
  \caption{SAA: Safe agreement for simulating steps of process A}
  \label{alg:SAA}
  \begin{algorithmic}[1]
    \Statex \textbf{shared variables} $R[1..n]$ array of $n$ 3-valued registers, initially $[\bot,\ldots,\bot]$   
    \Function{propose}{$v$}\label{saa:propose} \Comment{$v \in
      \{\mathtt{STOP},\mathtt{CONTINUE}, \mathtt{UNKNOWN}\}$}
    \State\label{saa:write_val}$R[i].\mathsf{write}(v)$ 
    \EndFunction
    \Function{decide}{$~$}\label{saa:decide}
    \State\label{saa:collect}$c \gets R.\mathsf{collect}()$;
    % \If{$\exists v \in \{\mathtt{STOP},\mathtt{CONTINUE}\} : \#_v(c) \geq  n-1$}\label{saa:return_val} \textsl{return} $v$ \EndIf
    \If{$\#_\bot(c) = 0$}
    \If{$\exists v \in
      \{\mathtt{STOP},\mathtt{CONTINUE}:\#_v(c)>0$}\label{saa:return_maj} \emph{return} the value
    $\in \{\mathtt{STOP},\mathtt{CONTINUE}\}$  with the largest number of
    occurrences in $c$, $\mathtt{STOP}$ in case of equality
    \Else{} \textsl{return} \texttt{UNKNOWN}\label{saa:return_unknown}
    \EndIf
    \Else{} \textsl{return}\label{saa:return_bot} $\bot$ \EndIf
    \EndFunction
  \end{algorithmic}
\end{algorithm}

Next lemma states the properties of algorithm~\ref{alg:SAA}. Thy
directly follow from the code. 
\begin{lemma}
  \label{lem:SAA}
  Algorithms~\ref{alg:SAA} satisfies agreement, termination,
  consistent decisions, validity of safe agreement and
  \begin{itemize}
  \item non triviality: if every process invokes $\textsc{propose}()$
    and each invocation terminates, only finitely many invocations of
    $\textsc{decide()}$  return $\bot$.
  \end{itemize}
\end{lemma}


Processes use instances of Algorithm~\ref{alg:SAB} to propose views
for process $B$. The algorithm is the  safe-agreement implementation
of \citetodo{imbsraynalithink} with a minor modification
$A$.



Algorithm~\ref{alg:SAB} is a standard safe-agreement algorithm (\citetodo{RAynalImbs}).
\begin{algorithm}
  \caption{SAB: Safe agreement for simulating steps of process B}
  \label{alg:SAB}
  \begin{algorithmic}[1]
    \Statex \textbf{shared variables} $R[1..n]$ array of $n$ 6-valued registers, initially $[\bot,\ldots,\bot]$   
    \Function{propose}{$v$}\label{sab:propose} \Comment{$v \in \{\mathtt{STOP},\mathtt{CONTINUE}\}$}
    \State\label{sab:write}$R[i].\mathsf{write}(v,1)$
    \State\label{sab:repeat}\textbf{repeat}  $c \gets R.\mathsf{collect}()$ \textbf{until} $\#_\bot(c) \leq 1$
    \State\label{sab:propose_collect}$c \gets R.\mathsf{collect}()$
    \If{$\exists j : c[j] = (*,2)$}\label{sab:write_v0} $R[j].\mathsf{write}(v,0)$
    \Else{}\label{sab:write_v2} $R[j].\mathsf{write}(v,2)$ \EndIf
    \EndFunction
    
    \Function{decide}{$~$}\label{sab:decide}
    \State\label{sab:decide_collect}$c \gets R.\mathsf{collect}()$;
    \If{$\forall j: 1 \leq j \leq n, c[j] \neq (*,1)$}\label{sab:return_nonbot} \textsl{return} $\left\{
      \begin{array}{l}
        \mathtt{STOP} ~\mbox{if  $\exists j : c[j] = (\mathtt{STOP},2)$} \\
        \mathtt{CONTINUE} ~\mbox{otherwise}
      \end{array}\right.$
    \Else{}\label{sab:return_bot} \textsl{return} $\bot$
    \EndIf
    \EndFunction
  \end{algorithmic}
\end{algorithm}

\begin{lemma}
  \label{lem:SAB}
  Algorithm~\ref{alg:SAB} satisfies agreement, validity, consistent
  reads of safe-agreement and
  \begin{itemize}
  \item Termination: 
  \item 
  \end{itemize}
\end{lemma}
\paragraph{The simulation}

%% TODO SAAr r >1  - View agreement

\begin{algorithm}
  \caption{Simulation. Code for process $i$ with input $x_i$}
  \label{alg:sim}
  \begin{algorithmic}[1]
    \Statex \textbf{shared variables} $I[1..n]$ array of input registers 
    \Statex\hspace{\algorithmicindent} $\mathit{SAA}_0$ (Algorithm~\ref{alg:IAA}), $\mathit{SAB}_0$ (Algorithm~\ref{alg:IAB}), 
    \Statex\hspace{\algorithmicindent} $SAA_{1,2,\ldots}$ (Algorithm~\ref{alg:SAA}), $SAB_{1,2,\ldots}$ (Algorithm~\ref{alg:SAB}) safe agreement objects
    \Begin
    \State\label{ABsim:write_input}$I[i].\mathsf{write}(x_i)$ \Comment{write input}
    \State\label{ABsim:IA_propose}$SAA_0.\mathsf{propose}(); SAB_0.\mathsf{propose}()$ \Comment{round $0$}
    \For{$r=1,\ldots,R$}\label{ABsim:for} \Comment{simulate at most $R$ rounds of $\m{A}_R$}
    \State\label{ABsim:hp_false}$has\_prop_A \gets \emph{false}$ \Comment{Has $i$ proposed a view for $A$ in round $r$?}
    \Repeat{}\label{ABsim:repeat} $d_A \gets SAA_{r-1}.\mathsf{decide}(); d_B \gets SAB_{r-1}.\mathsf{decide}()$
    \Statex\Comment{Check for progress in simulation of round $r-1$}
    \If{$d_A = \mathtt{STOP} \lor d_B = \mathtt{STOP}$}\label{ABsim:stop} \Comment{$A$ or $B$  decide in the simulated execution}
    \State\label{ABsim:call_decide1}\textbf{let} $P \in \{A,B\}: d_P \neq \bot$; \textsl{return}    \Call{decide}{$P,d_P,r-1$}  \EndIf
    \If{$d_A = \mathtt{CONTINUE} ~\land \neg has\_prop_A$}\label{ABsim:dA_cont} \Comment{Simulate one more round for $A$}
    \State\label{ABsim:propA}$v_A \gets \left\{
      \begin{array}{l}
        \mathtt{STOP} ~\mbox{if $d_B = \bot$} \\
        \mathtt{CONTINUE} ~\mbox{otherwise}
      \end{array}
    \right.$; $SAA_r.\mathsf{propose}(v_A)$; $has\_prop_A \gets \emph{true}$
    \EndIf
    \If{$d_B = \mathtt{CONTINUE}$}\label{ABsim:dB_cont} \Comment{Simulate one more round for $A$}
    \If{$\neg has\_prop_A \land d_A = \bot$}\label{ABsim:check_hp} \Comment{Avoid blocking $SAA_r$}
    \State\label{ABsim:prop_unknown}$SAA_r.\mathsf{propose}(\mathtt{UNKNOWN})$; $has\_prop_A \gets \emph{true}$
    \EndIf
    \State\label{ABsim:propB}$v_B \gets \left\{
      \begin{array}{l}
        \mathtt{STOP} ~\mbox{if $d_A = \bot$} \\
        \mathtt{CONTINUE} ~\mbox{otherwise}
      \end{array}
    \right.$; $SAB_r.\mathsf{propose}(v_B)$ 
    \EndIf
    \Until{$(SAA_r.\mathsf{decide}()$; $SAB_r.\mathsf{decide}()) \neq (\bot,\bot)$}\label{ABsim:until}
    \Statex\Comment{simulation of round $r$ for $A$ or $B$ completes }
    \EndFor
    \State\label{ABsim:decide_R}$d_A \gets SAA_R.\mathsf{decide}()$; $d_B \gets SAB_R.\mathsf{decide}()$;
    \Statex\Comment{Simulation of $R$ rounds for $A$ or/and $B$ has completed}
    \State\label{ABsim:call_decide2}\textbf{let} $P \in \{A,B\}: d_P \neq \bot$;   \textsl{return}  \Call{decide}{$P,d_P,R$}
    \End
    \Function{decide}{$P,d,\rho$}\label{ABsim:func_decide}
    \State\label{ABsim:letd}\textbf{let} $d_\epsilon$ be the value returned by $P$ in $\m{A}_R$ when it decides  at round $\rho$ with view $d$ assuming $A$ and $B$ inputs are $0$ and $1$ respectively
    \State\label{ABsim:X}$(X_A,X_B) \gets (SAA_0.\mathsf{decide}(),SAB_0.\mathsf{decide}())$ \Comment{Define the path in the task output}
    \Case{$d_{\epsilon} =0 ~~~~~~$}\label{ABsim:case_0} \textsl{return} $\delta(X_A)[i]$
    \StateCase{$0 < d_{\epsilon} < 1$}\label{ABsim:case_epsilon} \textbf{let} $(y_0, y_\epsilon, \ldots, y_{k\epsilon}, \ldots, y_1) = path(\delta(X_A),\delta(X_B))$;
   \State\label{ABsim:case_1}\hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent} \textsl{return} $\delta(y_{d_\epsilon})[i]$     %\Comment{$X_A$ is a full input vector and $X_B$ is a partial input vector}
    \StateCase{$d_\epsilon = 1~~~~~~$} \textsl{return} $\delta(X_B)[i]$
    \EndCase\label{ABsim:endcase}
    \EndFunction     
  \end{algorithmic}
\end{algorithm}

\begin{lemma}
  
\end{lemma}
\begin{lemma}[termination]
  \label{lem:ABsim_termination}
  Every non-faulty process invokes $\textsc{decide}()$. 
\end{lemma}
\begin{proof}
  The proof is by contradiction. Let us assume that there is an execution of Algorithm~\ref{alg:sim} in which some non-faulty process $p$ does not invokes $\textsc{decide}()$. Let us observe that if $p$ exits the $\mathbf{for}$ loop (line~\ref{ABsim:for}-line~\ref{ABsim:until}), then it invokes $\textsc{decide}$ at line~\ref{ABsim:call_decide2}. Note also that the invocations of $\mathsf{propose}()$ at line~\ref{ABsim:IA_propose} by $p$ terminates. Indeed, $SAA_0$ is implemented by Algorithm~\ref{alg:IAA} and therefore every invocation of $\mathsf{propose}()$ on it by a non-faulty process terminates (Lemma~\ref{lem:iaa}). $SAB_0$ is implemented by Algorithm~\ref{alg:IAB} and, since at least $n-1$ non-faulty processes invoke $\mathsf{propose}()$ on $SAB_0$, $p$'s invocation terminates. Thus $p$ enters but never exits  \textbf{for} loop.  

  
\end{proof}
\begin{proof}
  A process decides by calling $\textsc{decide}$ at line~\ref{ABsim:call_decide1} or at line~\ref{ABsim:call_decide2}. If process $i$ does not decide, the
\end{proof}

\begin{lemma}
  \label{lem:ABsim_}
\end{lemma}
% %%================== OLD VERSION =============================
% \begin{algorithm}
%   \caption{Simulation. Code for process $i$ with input $x_i$}
%   \label{alg:sim}
%   \begin{algorithmic}[1]
%     \Statex \textbf{shared variables} $I[1..n]$ array of input registers 
%     \Statex\hspace{\algorithmicindent} $\mathit{IAA}$ (Algorithm~\ref{alg:IAA}), $\mathit{IAB}$ (Algorithm~\ref{alg:IAB}) input agreements for $A$ and $B$
%     \Statex\hspace{\algorithmicindent} $SAA_{1,2,\ldots}$ (Algorithm~\ref{alg:SAA}), $SAB_{1,2,\ldots}$ (Algorithm~\ref{alg:SAB}) safe agreement objects
%     \Begin
%     \State\label{ABsim:write_input}$I[i].\mathsf{write}(x_i)$ \Comment{write input}
%     \State\label{ABsim:IA_propose}$IAA.\mathsf{propose}(); IAB.\mathsf{propose}()$ \Comment{round $0$}
%     \State\label{ABsim:IA_decide1}\textbf{repeat}    $d_A \gets IAA.\mathsf{decide}(); d_B \gets IAB.\mathsf{decide}()$
%     \textbf{until} $(d_A,d_B) \neq (\bot,\bot)$ 
%     \For{$r=1,\ldots,R$}\label{ABsim:for} \Comment{simulate at most $R$ rounds of $\m{A}_R$}
%     \State 
%     \If{$d_A \neq \bot$}\label{ABsim:dA} \Comment{simulate outcome for $A$ of round $r$ of $\m{A}_R$ (Algorithm~\ref{fig:alg2})}
%     \State\label{ABsim:SAA_propose} $SAA_r.\mathsf{propose}(v_A)$ where $v_A \gets \left\{
%       \begin{array}{l}
%         \mathtt{STOP} ~\mbox{if $d_B = \bot$} \\
%         \mathtt{CONTINUE} ~\mbox{otherwise}
%       \end{array}
%     \right.$
%     \EndIf
%     \If{$d_B \neq \bot$}\label{ABsim:dB} \Comment{simulate outcome for $B$ of round $r$ of $\m{A}_R$ (Algorithm~\ref{fig:alg2})}
%     \State\label{ABsim:SAB_propose} $SAB_1.\mathsf{propose}(v_B)$  where $v_B \gets \left\{
%       \begin{array}{l}
%         \mathtt{STOP} ~\mbox{if $d_A = \bot$} \\
%         \mathtt{CONTINUE} ~\mbox{otherwise}
%       \end{array}
%     \right.$
%     \EndIf
%     \State\label{ABsim:SA_decide} \textbf{repeat}  $d_A \gets SAA_1.\mathsf{decide}()$; $d_B \gets SAB_1.\mathsf{decide}()$ \textbf{until}
%     $(d_A,d_B) \neq (\bot,\bot)$
%     \If{$\mathtt{STOP} \in \{d_A,d_B\}$}\label{ABsim:break} \textsl{break} \EndIf
%     % \If{$d_P = \mathtt{STOP}$ for some $P \in \{A,B\}$} \textsl{break} \EndIf
%     \EndFor
%     \State\label{ABsim:letP} \textbf{let} $P \in \{A,B\}$ such that $d_P \neq \bot$;
%     \State\label{ABsim:letd} \textbf{let} $d_\epsilon$ be the value returned by $P$ in $\m{A}_R$ when it decides  at round $r$, assuming $A$ and $B$ inputs are $0$ and $1$ respectively 
%     \State\label{ABsim:IA_decide2} $(X_A,X_B) \gets (IAA.\mathsf{decide}(),IAB.\mathsf{decide}())$ \Comment{Define the path in the task output}
%     \Case{$d_{\epsilon} =0 ~~~~~~$}\label{ABsim:case_0} \textsl{return} $\delta(X_A)[i]$
%     \StateCase{$0 < d_{\epsilon} < 1$}\label{ABsim:case_epsilon} \textbf{let} $(y_0, y_\epsilon, \ldots, y_{k\epsilon}, \ldots, y_1) = path(\delta(X_A),\delta(X_B))$;
%     \State\label{ABsim:case_1}\hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent}\hspace{\algorithmicindent} \textsl{return} $\delta(y_{d_\epsilon})[i]$     %\Comment{$X_A$ is a full input vector and $X_B$ is a partial input vector}
%     \StateCase{$d_\epsilon = 1~~~~~~$}\label{ABsim:} \textsl{return} $\delta(X_B)[i]$
%     \EndCase
%     \End
%   \end{algorithmic}
% \end{algorithm}

\paragraph{Recycling safe agreement objects}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> linear_register.tex <==
\section{OLD SECTION : linear size registers are universal for $1 \leq t < \frac{n}{2}$}
\label{sec:t_larger_than_1}

\textbf{old result: linear size register are universal when $t < \frac{n}{2}$. We now have a slightly better result : registers only need to be of size $O(t)$ (the hidden constant does not depend on the task one wants to solve)}

We prove (Theorem~\ref{thm:linear_bounded})in this section that linear-bounded registers are universal as long as $t<\frac{n}{2}$. By contrast, when $t > \frac{n}{2}$, the size of the registers cannot be bounded. We show (Theorem~\ref{thm:no_dum}) for any bound $B:\mathbb{N} \to \mathbb{N}$, there is a task that cannot be solved tolerating by $n$ processes $t>\frac{n}{2}$ failures when the size of the registers is at most $B(n)$. 

\subsection{Universality of linear-bounded register for $t < \frac{n}{2}$}
\begin{theorem}
  \label{thm:linear_bounded}  \label{thm:majority}
  Let $T$ be a  task, $n,t$ be integers with $1 \leq t < \frac{n}{2}$.
  $T$ solvable with $n$ unbounded SWMR tolerating $t$ failures $\implies$ $t$ solvable with $n$ SWMR communication  registers of size $O(n)$ tolerating $t$ failures. 
\end{theorem}
% ========
% A METTRE EN SECTION 5 

% \begin{theorem}

%   Let $n,t, 1 < t < n/2$. 
%   For all  tasks $T$,
%   $T$ is solvable $t$-resilient by $n$ processes with  $n$ SWMR
%   registers if and only if $T$ is solvable $t$-resilient by $n$ processes with  $n$ SWMR registers of size $O(n)$.
% \end{theorem}


\begin{proof} (sketch)
Assume a task $T$ is solvable $t$-resilient by $n$ processes with  $n$ SWMR registers.
As $1<t<n/2$, by \cite{AttiyaBD95} it is possible to simulate registers in message passing. 
So $T$ is also solvable $t$-resilient by $n$ processes in message
passing. 

By standard and classical methods 
any  channel from $p$ to $q$ may be simulated by
a constant number of 1-bit SWSR registers  written and read by $p$ and
$q$.

We can for example proceed as follows.
First by an appropriate codage of messages, a channel between $p$ and $q$
with message of any size can be simulated
with a (FIFO) channel with messages of one bit.
Then such a channel may be
simulated by (1) one SWSR register $R_{p,q}$ written by $p$ 
and read by $q$ to transmit the data, (2) a SWSR register $S_{p,q}$ written by $p$
and read by $q$ and a SWSR register $S_{q,p}$ written by $q$ and read by $p$ to
synchronize $p$ and $q$.
On each register $S_{p,q}$ and $S_{q,p}$ the writer
alternates writing $0$ and $1$.
To transmit one bit $x$,  $p$ waits for
reading in $S_{q,p}$ a different bit from the previously bit read in
this register, writes $x$ in $R_{p,q}$ and writes a new bit (alternating $0$
and $1$) in $S_{p,q}$.
On the other hand, $q$ waits for reading in $S_{q,p}$ a different bit from the previously bit read in
this register, then reads $R_{p,q}$ the received bit, and  writes a new bit (alternating $0$
and $1$) in $S_{q,p}$.
For all $q$, registers  $R_{p,q}$ and $S_{p,q}$ are only written by
$p$, by an  appropriate codage with $O(n)$ bits it is possible to combine
them  in one $O(n)$ bits SWMR register (written by $p$).

Hence if $T$ is solvable $t$-resilient by $n$ processes with $n$ SWMR
registers of size $O(n)$.


% ----- ancienne version
% The messages that a process $p$ have to sent to a process $q$ are sent one by one.
% To send a message from process $p$ to process $q$, process $p$ sends the message bit per bit 
% and waits for an acknowledge of process $q$ before sending the next
% bit. This can be done with message of size $O(1)$. 
% So $T$ is solvable $t$-resilient by $n$ processes in message passing
% with message of size $O(1)$. 

% We can simulate the canal from $p$ to $q$, where $p$ sends  messages of size $s$
% by a SWSR register of size $s+1$  written by $p$ and read by $q$ 
% and a SWSR register of size 1 written by $q$ and read by $p$.
% To send a message $m$, the process $p$ writes  $m$ and a bit in the first register
% and it waits that process $q$ has written an acknowledgement (a bit) to the second register. 
% To receive a message the process $q$ reads the first register and
% writes an acknowledgement (a bit) in the second register. 
% To avoid to read twice the same message, the process $p$ alternates the bit that it writes with the message 
% and $q$ considers that it is a new message if the additional bit has changed.
% In the same way, to write the acknowledgement, the process $q$ alternates with 0 and 1.

% Each process uses $n-1$ SWSR registers of size $O(1)$ and $n-1$ SWSR registers of one bit for the acknowledgement
% This can be done in one SWMR of size $O(n)$.
% So $T$ is solvable $t$-resilient by $n$ processes with  $n$ SWMR registers of size $O(n)$.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

